Tracing OCaml Programs

This presentation will cover a framework for application-level tracing of OCaml programs. We outline a solution to the main technical challenge, which is being able to log typed values with lower overhead and maintenance burden than existing approaches. We then demonstrate the tools we have built around this for visualizing and exploring executions.

==> compile.tex <==
\begin{tikzpicture}
%%
\node (debug) at (35.747bp,80.0bp) [draw,rectangle] {debug.ml};
  \node (lib) at (218.29bp,116.0bp) [draw,rectangle] {lib.ml};
  \node (debugexe) at (218.29bp,56.0bp) [draw,ellipse] {debug.exe};
  \node (libcmt) at (405.09bp,94.0bp) [draw,ellipse] {lib.cmt};
  \node (app) at (35.747bp,145.0bp) [draw,ellipse] {app.ml};
  \node (appexe) at (218.29bp,170.0bp) [draw,ellipse] {app.exe};
  \node (debugtrace) at (405.09bp,159.0bp) [draw,ellipse] {debug.trace};
  \node (tracejson) at (405.09bp,18.0bp) [draw,ellipse] {trace.json};
  \draw [->] (debug) ..controls (101.37bp,92.885bp) and (148.66bp,102.31bp)  .. node[above, sloped] {depends on} (lib);
  \draw [->] (debug) ..controls (76.214bp,60.631bp) and (82.947bp,58.392bp)  .. (89.494bp,57.0bp) .. controls (113.02bp,51.998bp) and (139.53bp,51.053bp)  .. node[above, sloped] {compiles to} (debugexe);
  \draw [->] (lib) ..controls (271.37bp,116.59bp) and (312.22bp,115.64bp)  .. (347.09bp,110.0bp) .. controls (352.67bp,109.1bp) and (358.48bp,107.84bp)  .. node[above, sloped] {compiles to} (libcmt);
  \draw [->] (app) ..controls (75.164bp,135.79bp) and (82.561bp,134.25bp)  .. (89.494bp,133.0bp) .. controls (120.28bp,127.46bp) and (155.53bp,122.91bp)  .. node[above, sloped] {depends on} (lib);
  \draw [->] (app) ..controls (99.063bp,153.63bp) and (139.76bp,159.27bp)  .. node[above, sloped] {compiles to} (appexe);
  \draw [->] (appexe) ..controls (284.92bp,166.09bp) and (323.93bp,163.77bp)  .. node[above, sloped] {produces} (debugtrace);
  \draw [->] (debugexe) ..controls (294.11bp,75.162bp) and (343.41bp,88.211bp)  .. (347.09bp,91.0bp) .. controls (359.47bp,100.4bp) and (355.44bp,108.81bp)  .. (365.09bp,121.0bp) .. controls (368.53bp,125.36bp) and (372.45bp,129.71bp)  .. node[above, sloped] {reads} (debugtrace);
  \draw [->] (debugexe) ..controls (287.94bp,48.58bp) and (319.89bp,48.83bp)  .. (347.09bp,57.0bp) .. controls (357.96bp,60.266bp) and (368.71bp,66.306bp)  .. node[above, sloped] {reads} (libcmt);
  \draw [->] (debugexe) ..controls (259.76bp,38.088bp) and (271.76bp,33.774bp)  .. (283.09bp,31.0bp) .. controls (308.27bp,24.831bp) and (337.11bp,21.589bp)  .. node[above, sloped] {produces} (tracejson);
%
\end{tikzpicture}

